Recursive Polynomial Method for Fast Collision Avoidance Maneuver Design

A simple and reliable algorithm for collision avoidance maneuvers (CAMs), capable of computing impulsive, multi-impulsive, and low-thrust maneuvers, is proposed. The probability of collision (PoC) is approximated by a polynomial of arbitrary order as a function of the control, transforming the CAM designinto a polynomial program. The solution procedure is initiated by computing the CAM via a first-order greedy optimization approach, wherein the control action is applied in the direction of the gradient of PoC to maximize its change. Successively, the polynomial is truncated at higher orders, and the solution of the previous order is used to linearize the constraint. This enables achieving accurate solutions even for highly nonlinear safety metrics and dynamics. Since the optimization process comprises only polynomial evaluations, the method is computationally efficient, with run times typically below 1 s. Moreover, no restrictions on the considered dynamics are necessary; therefore, results are shown for Keplerian, J2, and circular restricted three-body problem dynamics.

==> Figures/B-plane.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,465); %set diagram left start at 0, and has height of 465

%Straight Lines [id:da1719990401256153] 
\draw [line width=1.5]  [dash pattern={on 5.63pt off 4.5pt}]  (370,238) -- (371,121.67) ;
%Straight Lines [id:da6056213587618334] 
\draw [line width=1.5]  [dash pattern={on 5.63pt off 4.5pt}]  (371,121.67) -- (282.75,87.5) ;
%Straight Lines [id:da21160951945207707] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.75]    (283,203) -- (236.77,29.9) ;
\draw [shift={(236,27)}, rotate = 75.05] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da7666646074688507] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=1.5]    (283,203) -- (368.06,124.38) ;
\draw [shift={(371,121.67)}, rotate = 137.25] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (11.61,-5.58) -- (0,0) -- (11.61,5.58) -- cycle    ;
%Straight Lines [id:da47921981090746657] 
\draw [line width=1.5]    (283,203) -- (408.29,253.5) ;
\draw [shift={(412,255)}, rotate = 201.95] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (11.61,-5.58) -- (0,0) -- (11.61,5.58) -- cycle    ;
%Shape: Circle [id:dp7100792087747478] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (364.33,121.67) .. controls (364.33,117.98) and (367.32,115) .. (371,115) .. controls (374.68,115) and (377.67,117.98) .. (377.67,121.67) .. controls (377.67,125.35) and (374.68,128.33) .. (371,128.33) .. controls (367.32,128.33) and (364.33,125.35) .. (364.33,121.67) -- cycle ;
%Straight Lines [id:da2872937414839446] 
\draw [line width=1.5]    (283,203) -- (139.87,240) ;
\draw [shift={(136,241)}, rotate = 345.51] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (11.61,-5.58) -- (0,0) -- (11.61,5.58) -- cycle    ;
%Straight Lines [id:da7614184023654675] 
\draw [line width=1.5]    (283,203) -- (283,33) ;
\draw [shift={(283,29)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (11.61,-5.58) -- (0,0) -- (11.61,5.58) -- cycle    ;
%Straight Lines [id:da5741149422048625] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.75]    (283,203) -- (149.98,52.25) ;
\draw [shift={(148,50)}, rotate = 48.58] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da6917854388377487] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=1.5]    (283,203) -- (198.87,224.99) ;
\draw [shift={(195,226)}, rotate = 345.35] [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (11.61,-5.58) -- (0,0) -- (11.61,5.58) -- cycle    ;
%Shape: Circle [id:dp8022912382599631] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (276.33,203) .. controls (276.33,199.32) and (279.32,196.33) .. (283,196.33) .. controls (286.68,196.33) and (289.67,199.32) .. (289.67,203) .. controls (289.67,206.68) and (286.68,209.67) .. (283,209.67) .. controls (279.32,209.67) and (276.33,206.68) .. (276.33,203) -- cycle ;
%Straight Lines [id:da21867553564150388] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=1.5]    (236,27) -- (151.87,48.99) ;
\draw [shift={(148,50)}, rotate = 345.35] [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (11.61,-5.58) -- (0,0) -- (11.61,5.58) -- cycle    ;

% Text Node
\draw (262.33,26) node [anchor=north west][inner sep=0.75pt]    {$\xi $};
% Text Node
\draw (383.33,250) node [anchor=north west][inner sep=0.75pt]    {$\zeta $};
% Text Node
\draw (151,240) node [anchor=north west][inner sep=0.75pt]    {$\eta $};
% Text Node
\draw (195,70) node [anchor=north west][inner sep=0.75pt]    {$\textcolor[rgb]{0.82,0.01,0.11}{\vec{v}_s(t_{CA})}$};
% Text Node
\draw (125,78) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$\textcolor[rgb]{0.29,0.56,0.89}{\vec{v}_p(t_{CA})}$};
% Text Node
\draw (343,125) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$\textcolor[rgb]{0.29,0.56,0.89}{\vec{r}}$};
% Text Node
\draw (160,28) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$\textcolor[rgb]{0.25,0.46,0.02}{\vec{v}}$};
% Text Node
\draw (210,225) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$\textcolor[rgb]{0.25,0.46,0.02}{\vec{v}}$};
% Text Node
\draw (249,213) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textcolor[rgb]{0.82,0.01,0.11}{Secondary}};
% Text Node
\draw (361,92) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textcolor[rgb]{0.29,0.56,0.89}{Primary}};


\end{tikzpicture}


==> glossary.tex <==
\newacronym{leo}{LEO}{low Earth orbit}
\newacronym{geo}{GEO}{geostationary Earth orbit}
\newacronym{smd}{SMD}{squared Mahalanobis distance}
\newacronym{ssa}{SSA}{Space Situational Awareness}
\newacronym{adr}{ADR}{Active Debris Removal}
\newacronym{sk}{SK}{station keeping}
\newacronym{ca}{CA}{collision avoidance}
\newacronym{ipc}{IPoC}{instantaneous probability of collision}
\newacronym{tipc}{TIPoC}{total instantaneous probability of collision}
\newacronym{cpc}{CPoC}{cumulative probability of collision}
\newacronym{poc}{PoC}{probability of collision}
\newacronym{tpoc}{TPoC}{total probability of collision}
\newacronym{cam}{CAM}{collision avoidance maneuver}
\newacronym{scvx}{SCvx}{successive convexification}
\newacronym{erf}{erf}{error function}
\newacronym{da}{DA}{differential algebra}
\newacronym{eci}{ECI}{Earth Centered Inertial}
\newacronym{ecef}{ECEF}{Earth Centered Earth Fixed}
\newacronym{lvlh}{LVLH}{Local Vertical Local Horizon}
\newacronym{hbr}{HBR}{hard body radius}
\newacronym{pdf}{PDF}{Probability Density Function}
\newacronym{nlp}{NLP}{nonlinear program}
\newacronym{srp}{SRP}{solar radiation pressure}
\newacronym{mpbvp}{MPBVP}{multi-point boundary value problem}
\newacronym{cw}{CW}{Clohessy-Wiltshire}
\newacronym{ns}{N-S}{North-South}
\newacronym{sdp}{SDP}{Semidefinite program}
\newacronym{qcqp}{QCQP}{Quadratically constrained quadratic program}
\newacronym{qp}{QP}{quadratic program}
\newacronym{zoh}{ZOH}{zeroth-order hold}
\newacronym{ocp}{OCP}{optimal control problem}
\newacronym{ew}{E-W}{East-West}
\newacronym{stm}{STM}{state transition matrix}
\newacronym{rtn}{RTN}{radial, along-track, cross-track}
\newacronym{iss}{ISS}{International Space Station}
\newacronym{lp}{LP}{linear program}
\newacronym{gnc}{GNC}{guidance, navigation, and control}
\newacronym{koz}{KOZ}{keep-out-zone}
\newacronym{socp}{SOCP}{second-order cone program}
\newacronym{cp}{CP}{convex program}
\newacronym{mrv}{MRV}{multivariate random variable}
\newacronym{gmm}{GMM}{Gaussian mixture model}
\newacronym{rv}{RV}{random variable}
\newacronym{scp}{SCP}{sequential convex program}
\newacronym{rso}{RSO}{resident space object}
\newacronym{mc}{MC}{Monte Carlo}
\newacronym{mss}{MSS}{Mahalanobis Shell Sampling}
\newacronym{nli}{NLI}{nonlinearity index}
\newacronym{rk}{RK}{Runge-Kutta}
\newacronym{trr}{TRR}{trust region radius}
\newacronym{tca}{TCA}{time of closest approach}
\newacronym{gto}{GTO}{Geostationary Transfer Orbit}
\newacronym{aida}{AIDA}{Accurate Integrator for Debris Analysis}
\newacronym{ava}{AvA}{active vs active}
\newacronym{cdm}{CDM}{Conjunction Data Message}
\newacronym{cr3bp}{CR3BP}{circular restricted three-body problem}
\newacronym{pp}{PP}{polynomial program}
\newacronym{stt}{STT}{state transition tensor}

